Learning to Find Proofs and Theorems by Learning to Refine Search Strategies: The Case of Loop Invariant Synthesis

We propose a new approach to automated theorem proving where an AlphaZero-style agent is self-training to refine a generic high-level expert strategy expressed as a nondeterministic program. An analogous teacher agent is self-training to generate tasks of suitable relevance and difficulty for the learner. This allows leveraging minimal amounts of domain knowledge to tackle problems for which training data is unavailable or hard to synthesize. As a specific illustration, we consider loop invariant synthesis for imperative programs and use neural networks to refine both the teacher and solver strategies.

==> content/teacher-strategy.tex <==
\noindent\begin{minipage}[t]{.5\columnwidth}
  \begin{lstlisting}[
    language=Python,
    numbers=left,
    xleftmargin=\lstleftmargin
  ]
  def teacher():

      prog: Prog = "
          init;
          while (guard) {
              invariant inv;
              body;
          }
          assert post;"

      checkpoint();
      refine('guard', ['cbound', 'vcomp', '??'])
      instantiate_consts()
      extra = relax_ineq('guard')
      refine_conj('inv', [
          ['cbound', 'vcomp', 'linear', extra],
          ['cbound', extra], ['cbound']])
      assert sat("$inv")
      if choose([True, False]):
          refine('inv', "$inv || $guard")
      instantiate_consts()
      assert not valid("$inv -> $guard")

      checkpoint()
      refine_body()
      abduct_consts(
          "$guard & $inv -> wlp($body, $inv)")
      instantiate_consts()

      checkpoint()
      common = ['cbound', 'vcomp', 'eq']
      extra = consequences("!$guard & $inv")
      refine_disj('post',
          common + ['lin'] + extra,
          common)
      abduct_consts("!$guard & $inv -> $post")
      instantiate_consts()
      assert not valid("!$guard -> $post")

      checkpoint()
      instantiate_init()
      abduct_consts("wlp($init, $inv)")
      instantiate_consts()
      assert sat("wlp($init, $gurd)")
      assert not valid("wlp($init, false)")

      split_double_assumptions(prog)
      move_param_assums(prog)
      shuffle_post(prog)
      reformat_post(prog)
      params_to_vars(prog)
      shuffle_comparisons(prog)
      remove_invariant(prog)
      return prog
  \end{lstlisting}
  \end{minipage}\hfill
  \begin{minipage}[t]{.47\columnwidth}
  \begin{lstlisting}[
    language=Python,
    numbers=left,
    xleftmargin=\lstleftmargin,
    firstnumber=last
  ]
      def refine(fml, templates):
          x, y, z = fresh_var_holes(3)
          c = fresh_const(1)
          choices = []
          for t in templates:
              if t == 'cbound':
                  choices += [
                      "x<=c", "x<c",
                      "x>=c", "x>c"
              if t == 'vcomp':
                  choices += ["x>=y+c"]
              if t == '??':
                  choices += ["??"]
              if t == 'eq':
                  choices += ["x=c, x=y"]
              if t == 'neq':
                  choices += ["x!=c, x!=y"]
              if t == 'lin':
                  choices += [
                      "$(random_lin([x,y])) = c",
                      "$(random_lin([x,y])) >= c",
                      "$(random_lin([x,y,z])) = c"]
              if isinstance(t, Formula):
                  choices += [t]
          refine(fml, choose(choices))
          instantiate_dyn_vars()
  \end{lstlisting}
  \end{minipage}


==> figures/intro-solver-example.tex <==
\begin{figure}
    \begin{subfigure}{0.7\textwidth}
      \centering
      \input{content/simplified-solver.tex}
      \caption{Solver strategy}
    \end{subfigure}
    \begin{subfigure}{0.25\textwidth}
      \begin{subfigure}{\textwidth}
        \centering
        \input{content/example-prog.tex}
        \caption{Example program}
      \end{subfigure}\\[5ex]
      \begin{subfigure}{\textwidth}
        \centering
        \[x \ge y \ \wedge\  x \ge 1 \ \wedge \ y \ge 0 \]
        \caption{Invariant}
      \end{subfigure}
    \end{subfigure}
  \caption{A simplified solver strategy for loop invariant generation}
\end{figure}

% \begin{wrapfigure}{r}{0.35\textwidth}
%   \begin{center}
%     \begin{minipage}{0.21\textwidth}
%       \setlstc{}
%       \input{content/example-prog.tex}
%     \end{minipage}
%   \end{center}
%   \caption{An example program}
% \end{wrapfigure}

==> figures/simplified-solver.tex <==
\begin{wrapfigure}{l}{0.6\textwidth}
  \setlstpy{}
  \begin{minipage}{0.6\textwidth}
    \input{content/simplified-solver.tex}
  \end{minipage}
  \caption{Simplified solver strategy.}\label{fig:solver-simplified}
\end{wrapfigure}

==> generated/hyperparams.tex <==
\\ \toprule
\textbf{Parameter} & \textbf{Value} & \textbf{Description} \\ \toprule
\texttt{params} &   & \pbox[c]{6cm}{All hyperparameters.} \\ \midrule
\ {\tiny *} \  \texttt{teacher} &   & \pbox[c]{6cm}{Hyperparameters for the teacher agent.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \texttt{agent} &   & \pbox[c]{6cm}{Hyperparameters common to all AlphaZero agents.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-iters} & \pbox[c]{1.2cm}{20} & \pbox[c]{6cm}{Total number of training iterations.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-problems-per-iter} & \pbox[c]{1.2cm}{8000} & \pbox[c]{6cm}{Number of data generation episodes per iteration.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-validation-problems} & \pbox[c]{1.2cm}{800} & \pbox[c]{6cm}{Number of validation-data generation episodes per iteration.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-workers} & \pbox[c]{1.2cm}{600} & \pbox[c]{6cm}{Number of episodes simulated in parallel or asynchronously during data generation.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-processes} & \pbox[c]{1.2cm}{none} & \pbox[c]{6cm}{Number of distinct CPU processes spawned for data generation (by default, this value is set to the number of available physical CPU cores).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{search} &   & \pbox[c]{6cm}{Proof search limits.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-proof-length} & \pbox[c]{1.2cm}{60} & \pbox[c]{6cm}{Maximum number of allowed environment steps before failing automatically.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-probe-size} & \pbox[c]{1.2cm}{80} & \pbox[c]{6cm}{Maximum allowed size of state encodings. Bigger state encodings result in immediate failures.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-action-size} & \pbox[c]{1.2cm}{12} & \pbox[c]{6cm}{Maximum allowed size of action encodings. Actions with bigger encodings are discarded.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{encoding} &   & \pbox[c]{6cm}{State and action encoding hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{d-model} & \pbox[c]{1.2cm}{128} & \pbox[c]{6cm}{Embedding size for tokens, which is also equal to the neural network's state dimension.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{pos-enc-size} & \pbox[c]{1.2cm}{32} & \pbox[c]{6cm}{Maximal size of the tree positional encoding added to each token embedding.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{uid-emb-size} & \pbox[c]{1.2cm}{16} & \pbox[c]{6cm}{Maximum number of unique identifiers that can be encoded.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{const-emb-size} & \pbox[c]{1.2cm}{0} & \pbox[c]{6cm}{Maximum number of bits used to encode the binary value of numerical constants. No encoding is done if a value of 0 is provided.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{enable-numerical-edges} & \pbox[c]{1.2cm}{true} & \pbox[c]{6cm}{Add comparison edges between numerical constants.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{add-reverse-edges} & \pbox[c]{1.2cm}{true} & \pbox[c]{6cm}{Add reverse edges for all edge types.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{network} &   & \pbox[c]{6cm}{Hyperparameters for the Dynamic Graph Transformer network.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-heads} & \pbox[c]{1.2cm}{4} & \pbox[c]{6cm}{Number of transformer attention heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{probe-encoder-layers} & \pbox[c]{1.2cm}{6} & \pbox[c]{6cm}{Number of transformer blocks used to encode states.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{action-encoder-layers} & \pbox[c]{1.2cm}{3} & \pbox[c]{6cm}{Number of transformer blocks used to encode actions} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{combiner-layers} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Number of transformer blocks used in the combiner network that combines state and action encodings.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dropout-rate} & \pbox[c]{1.2cm}{0.05} & \pbox[c]{6cm}{Dropout rate.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-head-layers} & \pbox[c]{1.2cm}{2} & \pbox[c]{6cm}{Number of layers in the feed-forward networks used for the value and policy heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{head-dim} & \pbox[c]{1.2cm}{256} & \pbox[c]{6cm}{Hidden dimension of layers in the feed-forward networks used for the value and policy heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{mcts} &   & \pbox[c]{6cm}{MCTS hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-simulations} & \pbox[c]{1.2cm}{64} & \pbox[c]{6cm}{Number of MCTS simulations used for planning every environment step.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-considered-actions} & \pbox[c]{1.2cm}{8} & \pbox[c]{6cm}{The number of top-ranked actions that are considered in the sequential halving Gumbel exploration process.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{value-scale} & \pbox[c]{1.2cm}{0.1} & \pbox[c]{6cm}{The $c_{\text{scale}}$ hyperparameter (see original Gumbel AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-visit-init} & \pbox[c]{1.2cm}{50} & \pbox[c]{6cm}{The $c_{\text{visit}}$ hyperparameter (see original Gumbel AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{fpu-red} & \pbox[c]{1.2cm}{0.1} & \pbox[c]{6cm}{Value estimates for unvisited children are decreased by this value so as to encourage deeper search trees (see LC0 AlphaZero implementation).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{reset-tree} & \pbox[c]{1.2cm}{true} & \pbox[c]{6cm}{Whether the MCTS tree is reset after an environment move is taken.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-tree-size} & \pbox[c]{1.2cm}{256} & \pbox[c]{6cm}{Maximal size of the MCTS tree. This parameter is relevant to avoid out-of-memory errors when \texttt{reset-tree} if false.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dirichlet-alpha} & \pbox[c]{1.2cm}{10} & \pbox[c]{6cm}{Concentration parameter for the Dirichlet exploration noise (see original AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dirichlet-eps} & \pbox[c]{1.2cm}{0.25} & \pbox[c]{6cm}{Magnitude of the Dirichlet exploration noise. No Dirichlet exploration noise is normally used with Gumbel AlphaZero but we add some anyway in the teacher for increased diversity.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{training} &   & \pbox[c]{6cm}{Network training hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-epochs} & \pbox[c]{1.2cm}{6} & \pbox[c]{6cm}{The maximum number of training epochs.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{improvement-required} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Gradient updates are stopped if the validation loss fails to decrease for more than this number of epochs.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{batch-size} & \pbox[c]{1.2cm}{400} & \pbox[c]{6cm}{Training batch size.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{lr-base} & \pbox[c]{1.2cm}{0.0005} & \pbox[c]{6cm}{Maximal learning rate used in a cosine learning rate schedule with warm-up.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{warmup-epochs} & \pbox[c]{1.2cm}{0.2} & \pbox[c]{6cm}{Length of the warm-up part of the learning rate schedule (in epochs).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{weight-decay} & \pbox[c]{1.2cm}{0.01} & \pbox[c]{6cm}{Weight decay parameter.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{outcome-loss-coeff} & \pbox[c]{1.2cm}{0.7} & \pbox[c]{6cm}{Coefficient for the loss term evaluating outcome prediction accuracy (e.g. success or failure).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{event-loss-coeff} & \pbox[c]{1.2cm}{3} & \pbox[c]{6cm}{Coefficient for the loss term evaluating event prediction accuracy.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{policy-loss-coeff} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Coefficient for the loss term evaluating the divergence from policy priors to their targets.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{training-window} & \pbox[c]{1.2cm}{1, 2, 2, 3, 3, 3, 4, 4, 4, 5, 5, 5, 6, 6, 6, 7} & \pbox[c]{6cm}{The number of previous iterations from which samples are used to update the network at each iteration. If the provided list is shorter than the total number of iterations, the last number in this list is duplicated as many times as necessary.} \\ \midrule
\ {\tiny *} \  \texttt{solver} &   & \pbox[c]{6cm}{Hyperparameters for the solver agent.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \texttt{agent} &   & \pbox[c]{6cm}{Hyperparameters common to all AlphaZero agents.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-iters} & \pbox[c]{1.2cm}{20} & \pbox[c]{6cm}{Total number of training iterations.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-problems-per-iter} & \pbox[c]{1.2cm}{20000} & \pbox[c]{6cm}{Number of data generation episodes per iteration.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-validation-problems} & \pbox[c]{1.2cm}{5000} & \pbox[c]{6cm}{Number of validation-data generation episodes per iteration.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-workers} & \pbox[c]{1.2cm}{600} & \pbox[c]{6cm}{Number of episodes simulated in parallel or asynchronously during data generation.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-processes} & \pbox[c]{1.2cm}{none} & \pbox[c]{6cm}{Number of distinct CPU processes spawned for data generation (by default, this value is set to the number of available physical CPU cores).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{search} &   & \pbox[c]{6cm}{Proof search limits.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-proof-length} & \pbox[c]{1.2cm}{12} & \pbox[c]{6cm}{Maximum number of allowed environment steps before failing automatically.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-probe-size} & \pbox[c]{1.2cm}{80} & \pbox[c]{6cm}{Maximum allowed size of state encodings. Bigger state encodings result in immediate failures.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-action-size} & \pbox[c]{1.2cm}{12} & \pbox[c]{6cm}{Maximum allowed size of action encodings. Actions with bigger encodings are discarded.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{encoding} &   & \pbox[c]{6cm}{State and action encoding hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{d-model} & \pbox[c]{1.2cm}{128} & \pbox[c]{6cm}{Embedding size for tokens, which is also equal to the neural network's state dimension.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{pos-enc-size} & \pbox[c]{1.2cm}{32} & \pbox[c]{6cm}{Maximal size of the tree positional encoding added to each token embedding.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{uid-emb-size} & \pbox[c]{1.2cm}{16} & \pbox[c]{6cm}{Maximum number of unique identifiers that can be encoded.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{const-emb-size} & \pbox[c]{1.2cm}{0} & \pbox[c]{6cm}{Maximum number of bits used to encode the binary value of numerical constants. No encoding is done if a value of 0 is provided.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{enable-numerical-edges} & \pbox[c]{1.2cm}{true} & \pbox[c]{6cm}{Add comparison edges between numerical constants.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{add-reverse-edges} & \pbox[c]{1.2cm}{true} & \pbox[c]{6cm}{Add reverse edges for all edge types.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{network} &   & \pbox[c]{6cm}{Hyperparameters for the Dynamic Graph Transformer network.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-heads} & \pbox[c]{1.2cm}{4} & \pbox[c]{6cm}{Number of transformer attention heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{probe-encoder-layers} & \pbox[c]{1.2cm}{6} & \pbox[c]{6cm}{Number of transformer blocks used to encode states.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{action-encoder-layers} & \pbox[c]{1.2cm}{3} & \pbox[c]{6cm}{Number of transformer blocks used to encode actions} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{combiner-layers} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Number of transformer blocks used in the combiner network that combines state and action encodings.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dropout-rate} & \pbox[c]{1.2cm}{0.1} & \pbox[c]{6cm}{Dropout rate.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-head-layers} & \pbox[c]{1.2cm}{2} & \pbox[c]{6cm}{Number of layers in the feed-forward networks used for the value and policy heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{head-dim} & \pbox[c]{1.2cm}{256} & \pbox[c]{6cm}{Hidden dimension of layers in the feed-forward networks used for the value and policy heads.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{mcts} &   & \pbox[c]{6cm}{MCTS hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-simulations} & \pbox[c]{1.2cm}{32} & \pbox[c]{6cm}{Number of MCTS simulations used for planning every environment step.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{num-considered-actions} & \pbox[c]{1.2cm}{8} & \pbox[c]{6cm}{The number of top-ranked actions that are considered in the sequential halving Gumbel exploration process.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{value-scale} & \pbox[c]{1.2cm}{0.1} & \pbox[c]{6cm}{The $c_{\text{scale}}$ hyperparameter (see original Gumbel AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-visit-init} & \pbox[c]{1.2cm}{50} & \pbox[c]{6cm}{The $c_{\text{visit}}$ hyperparameter (see original Gumbel AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{fpu-red} & \pbox[c]{1.2cm}{0} & \pbox[c]{6cm}{Value estimates for unvisited children are decreased by this value so as to encourage deeper search trees (see LC0 AlphaZero implementation).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{reset-tree} & \pbox[c]{1.2cm}{false} & \pbox[c]{6cm}{Whether the MCTS tree is reset after an environment move is taken.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-tree-size} & \pbox[c]{1.2cm}{256} & \pbox[c]{6cm}{Maximal size of the MCTS tree. This parameter is relevant to avoid out-of-memory errors when \texttt{reset-tree} if false.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dirichlet-alpha} & \pbox[c]{1.2cm}{10} & \pbox[c]{6cm}{Concentration parameter for the Dirichlet exploration noise (see original AlphaZero paper).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{dirichlet-eps} & \pbox[c]{1.2cm}{none} & \pbox[c]{6cm}{Magnitude of the Dirichlet exploration noise. No Dirichlet exploration noise is normally used with Gumbel AlphaZero but we add some anyway in the teacher for increased diversity.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{training} &   & \pbox[c]{6cm}{Network training hyperparameters.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{max-epochs} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{The maximum number of training epochs.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{improvement-required} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Gradient updates are stopped if the validation loss fails to decrease for more than this number of epochs.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{batch-size} & \pbox[c]{1.2cm}{300} & \pbox[c]{6cm}{Training batch size.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{lr-base} & \pbox[c]{1.2cm}{0.0003} & \pbox[c]{6cm}{Maximal learning rate used in a cosine learning rate schedule with warm-up.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{warmup-epochs} & \pbox[c]{1.2cm}{0.2} & \pbox[c]{6cm}{Length of the warm-up part of the learning rate schedule (in epochs).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{weight-decay} & \pbox[c]{1.2cm}{0.01} & \pbox[c]{6cm}{Weight decay parameter.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{outcome-loss-coeff} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Coefficient for the loss term evaluating outcome prediction accuracy (e.g. success or failure).} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{event-loss-coeff} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Coefficient for the loss term evaluating event prediction accuracy.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{policy-loss-coeff} & \pbox[c]{1.2cm}{1} & \pbox[c]{6cm}{Coefficient for the loss term evaluating the divergence from policy priors to their targets.} \\ \midrule
\ {\tiny *} \  \ {\tiny *} \  \ {\tiny *} \  \texttt{training-window} & \pbox[c]{1.2cm}{1, 2, 2, 3, 3, 3, 4, 4, 4, 5, 5, 5, 6, 6, 6, 7} & \pbox[c]{6cm}{The number of previous iterations from which samples are used to update the network at each iteration. If the provided list is shorter than the total number of iterations, the last number in this list is duplicated as many times as necessary.} \\ \midrule
\ {\tiny *} \  \texttt{num-teacher-iters-used-by-solver} & \pbox[c]{1.2cm}{5} & \pbox[c]{6cm}{The number of teacher training iterations from which solver training samples are collected.} \\ \midrule
\ {\tiny *} \  \texttt{extra-teacher-problems} & \pbox[c]{1.2cm}{10000} & \pbox[c]{6cm}{Number of extra teacher problems that are generated once the teacher is trained, with no exploration noise.} \\ \midrule
\bottomrule

